Enhancing Accuracy and Parameter-Efficiency of Neural Representations for Network Parameterization

In this work, we investigate the fundamental trade-off regarding accuracy and parameter efficiency in the parameterization of neural network weights using predictor networks. We present a surprising finding that, when recovering the original model accuracy is the sole objective, it can be achieved effectively through the weight reconstruction objective alone. Additionally, we explore the underlying factors for improving weight reconstruction under parameter-efficiency constraints, and propose a novel training scheme that decouples the reconstruction objective from auxiliary objectives such as knowledge distillation that leads to significant improvements compared to state-of-the-art approaches. Finally, these results pave way for more practical scenarios, where one needs to achieve improvements on both model accuracy and predictor network parameter-efficiency simultaneously.

==> body/framework.tex <==
% \section{Param-Distil: Knowledge Distillation with Parameterized Weights \Hongjun{NeRD as title suggested?}}
\section{Practical Usages for Weight Parameterization}
\label{sec:framework}
The proposed two stage training allows for more freedom in exploring solutions, as evidenced by the higher weight difference shown in Figure \ref{NeRN_Decoupling}(b). 
%%%%%
This observation also means we can effectively transfer the knowledge from the teacher network to the reconstructed weights via the predictor network. This represent a distinct perspective for approach the knowledge distillation problem as existing methods directly train the target network that often with small capacity, therefore, limited ability to learn. Through the introduction of a predictor network we can potentially significantly increase its capability without affecting the output network size. 
%
More importantly, as illustrated in Figure \ref{fig:proposed_approach}, the such a separation allow us to introduce high-capacity teacher network, and by pairing with a powerful predictor network, we can trade the additional computation cost and size for a smaller and better performing reconstructed network achieving meaningful inference time compression.

\begin{figure*}[htb!]
	\centering
	\includegraphics[width=0.90\linewidth]{Figures/Section3_Fig_NeRN_Decoupling.png}
	\caption{Overview of the proposed framework. We decoupling the training objectives into two distinct phases: a reconstruction phase and a distillation phase. During the distillation phase, a high-capacity teacher network, pre-trained beforehand, is employed to provide additional guidance.}\label{fig:proposed_approach}
% \vspace{-1.0em}
\end{figure*}

% While it is feasible to train both phases sequentially using a learning rate schedule, we consider a more general scenario where pre-trained Recon-NeRNs are available. 
Specifically, fully separating the two phases offers the advantage of enabling more flexible learning during the fine-tuning stage of the second phase. For example, this facilitates the exploration of different optimizers compared to those used in the first phase. Additionally, to maximize the performance of the predictor network, it allows for the application of various advanced distillation methods that have been previously explored. 
We show that with our proposed strategy, predicted network's performance can be significantly enhanced when distillation is provided by the high-quality predictive power from high-capacity teacher networks in the second phase. 
% Particularly, in contrast with baseline that use joint objectives cannot benefit from this superior supervision.




